Cascade production in the reactions gamma p --> K+ K+ (X) and gamma p --> K^+ K^+ pi- (X)

Photoproduction of the cascade resonances has been investigated in the reactions $\gamma p \to K^+ K^+ (X)$ and $\gamma p \to K^+ K^+ \pi^- (X)$. The mass split of the $\Xi$ doublet is measured to be $5.4\pm 1.8$ MeV/c$^2$, consistent with existing measurements. The differential (total) cross sections for the $\Xi^{-}$ have been determined for photon beam energies from 2.75 to 3.85 (4.75) GeV, and are consistent with a possible production mechanism of $Y^*\to K^+\Xi^-$ through a $t$-channel process. The reaction $\gamma p \to K^+ K^+ \pi^-[\Xi^0]$ has also been investigated in search of excited cascade resonances. No significant signal of excited cascade states other than the $\Xi^-(1530)$ is observed. The cross section results of the $\Xi^-(1530)$ have also been obtained for photon beam energies from 3.35 to 4.75 GeV.

==> memb_new.tex <==
% File   Generated 2003-7-13
%%%  
  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% FOLLOWING A GENERIC HEADER FOR TEX
%   nothing here relates to author list
%   may be deleted or replace by more updated code.
 
% Based on RevTEX4

%%%\documentclass[prl,superscriptaddress,showpacs,amssymb,amsmath,amsfonts,aps]{revtex4}
%% \setlength{\topmargin}{-1.0cm}
%% \usepackage{graphicx}
%% \usepackage{dcolumn}
%%%\begin{document}
%%%\title{{\large DRAFT: Author List}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% include other start up commands 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% List of authors
% Generated from the clas database. 
% Concerns about content related to future author lists email clasmbr@jlab.org 
% Concerns about content related to this publication must be sent to first authors
%   While writers of a publication will start with this list,
%   they maintain their own corrected verions as part of the developing publication.
% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% commands
%   define a shorthand notation XXX for affiliation names and addresses  
%      \newcommand*{\XXX}{Name, Address}
%   use the new commands
%        \affiliation{\XXX}     standard 
%        \altaffiliation{\XXX}  current address if different from above 
% to add the University and address information to each author
%  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% 
% 
% 
% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% 
%  date generated 2003-7-13
% 
% List is based on a time range  
%    start boundary 1=          Mon Jun 01 00:00:22 EDT 1998
%    end boundary 1  =          Sun Jun 28 00:00:22 EDT 1998
%    start boundary 2=          Thu Jul 01 00:00:22 EDT 1999
%    end boundary 2  =          Sat Jul 31 00:00:22 EDT 1999
% Full and Term members (and recent term) within the data recording period are made authors
% 
% Last window is the current members time window
% Including all term members that are currently members (term authorship bylaw)
% 
% Limited members are the responsibility of the first authors of the paper
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% Database contains a list of periods for each person  
%    If a person is found to be a full or term member 
%    then the affiliations at that time are listed 
%
%    The current affliation is checked if it is different from 
%    the affiliations listed then a current location is added
%  The publication status is checked. Some people are not interested
%    in any CLAS pubs and this is recorded in the database.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%% Institutes Number and defintions %%%%%%%%%%%
 
% FIRST time through establishes the order
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\newcommand*{\RPI }{ Rensselaer Polytechnic Institute, Troy, New York 12180-3590} 
\affiliation{\RPI } 

\newcommand*{\VANDER }{ Vanderbilt University, Nashville, Tennessee 37235}
\affiliation{\VANDER } 

\newcommand*{\JLAB }{ Thomas Jefferson National Accelerator Facility, Newport News, Virginia 23606} 
\affiliation{\JLAB } 

\newcommand*{\ASU }{ Arizona State University, Tempe, Arizona 85287-1504} 
\affiliation{\ASU } 

\newcommand*{\SACLAY }{ CEA-Saclay, Service de Physique Nucl\'eaire, F91191 Gif-sur-Yvette, Cedex, France} 
\affiliation{\SACLAY } 

\newcommand*{\UCLA }{ University of California at Los Angeles, Los Angeles, California  90095-1547} 
\affiliation{\UCLA } 

\newcommand*{\CMU }{ Carnegie Mellon University, Pittsburgh, Pennsylvania 15213} 
\affiliation{\CMU } 

\newcommand*{\CUA }{ Catholic University of America, Washington, D.C. 20064} 
\affiliation{\CUA } 

\newcommand*{\CNU }{ Christopher Newport University, Newport News, Virginia 23606} 
\affiliation{\CNU } 

\newcommand*{\UCONN }{ University of Connecticut, Storrs, Connecticut 06269} 
\affiliation{\UCONN } 

\newcommand*{\DUKE }{ Duke University, Durham, North Carolina 27708-0305} 
\affiliation{\DUKE } 

\newcommand*{\ECOSSEE }{ Edinburgh University, Edinburgh EH9 3JZ, United Kingdom} 
\affiliation{\ECOSSEE } 

\newcommand*{\FIU }{ Florida International University, Miami, Florida 33199} 
\affiliation{\FIU } 

\newcommand*{\FSU }{ Florida State University, Tallahassee, Florida 32306} 
\affiliation{\FSU } 

\newcommand*{\GWU }{ The George Washington University, Washington, DC 20052} 
\affiliation{\GWU } 

\newcommand*{\ECOSSEG }{ University of Glasgow, Glasgow G12 8QQ, United Kingdom} 
\affiliation{\ECOSSEG } 

\newcommand*{\INFNFR }{ INFN, Laboratori Nazionali di Frascati, Frascati, Italy} 
\affiliation{\INFNFR } 

\newcommand*{\INFNGE }{ INFN, Sezione di Genova, 16146 Genova, Italy} 
\affiliation{\INFNGE } 

\newcommand*{\ORSAY }{ Institut de Physique Nucleaire ORSAY, Orsay, France} 
\affiliation{\ORSAY } 

\newcommand*{\BONN }{ Institute f\"{u}r Strahlen und Kernphysik, Universit\"{a}t Bonn, Germany} 
\affiliation{\BONN } 

\newcommand*{\ITEP }{ Institute of Theoretical and Experimental Physics, Moscow, 117259, Russia} 
\affiliation{\ITEP } 

\newcommand*{\JMU }{ James Madison University, Harrisonburg, Virginia 22807} 
\affiliation{\JMU } 

\newcommand*{\KYUNGPOOK }{ Kungpook National University, Taegu 702-701, South Korea} 
\affiliation{\KYUNGPOOK } 

\newcommand*{\MIT }{ Massachusetts Institute of Technology, Cambridge, Massachusetts  02139-4307} 
\affiliation{\MIT } 

\newcommand*{\UMASS }{ University of Massachusetts, Amherst, Massachusetts  01003} 
\affiliation{\UMASS } 

\newcommand*{\UNH }{ University of New Hampshire, Durham, New Hampshire 03824-3568} 
\affiliation{\UNH } 

\newcommand*{\NSU }{ Norfolk State University, Norfolk, Virginia 23504} 
\affiliation{\NSU } 

\newcommand*{\OHIOU }{ Ohio University, Athens, Ohio  45701} 
\affiliation{\OHIOU } 

\newcommand*{\ODU }{ Old Dominion University, Norfolk, Virginia 23529} 
\affiliation{\ODU } 

\newcommand*{\PITT }{ University of Pittsburgh, Pittsburgh, Pennsylvania 15260} 
\affiliation{\PITT } 

\newcommand*{\ROMA }{ Universita' di ROMA III, 00146 Roma, Italy} 
\affiliation{\ROMA } 


\newcommand*{\RICE }{ Rice University, Houston, Texas 77005-1892} 
\affiliation{\RICE } 

\newcommand*{\URICH }{ University of Richmond, Richmond, Virginia 23173} 
\affiliation{\URICH } 

\newcommand*{\SCAROLINA }{ University of South Carolina, Columbia, South Carolina 29208} 
\affiliation{\SCAROLINA } 

\newcommand*{\UTEP }{ University of Texas at El Paso, El Paso, Texas 79968} 
\affiliation{\UTEP } 


\newcommand*{\UNIONC }{ Department of Physics, Schenectady, NY 12308} 
\affiliation{\UNIONC } 

\newcommand*{\VT }{ Virginia Polytechnic Institute and State University, Blacksburg, Virginia   24061-0435} 
\affiliation{\VT } 

\newcommand*{\VIRGINIA }{ University of Virginia, Charlottesville, Virginia 22901} 
\affiliation{\VIRGINIA } 

\newcommand*{\WM }{ College of William and Mary, Williamsburg, Virginia 23187-8795} 
\affiliation{\WM } 

\newcommand*{\YEREVAN }{ Yerevan Physics Institute, 375036 Yerevan, Armenia} 
\affiliation{\YEREVAN } 


%\newcommand*{\NONE }{ unknown} 
%\affiliation{\NONE } 

\newcommand*{\NOWNCATU }{ North Carolina Agricultural and Technical State University, Greensboro, NC 27411}

\newcommand*{\NOWECOSSEG }{ University of Glasgow, Glasgow G12 8QQ, United Kingdom}

\newcommand*{\NOWJLAB }{ Thomas Jefferson National Accelerator Facility, Newport News, Virginia 23606}

\newcommand*{\NOWSCAROLINA }{ University of South Carolina, Columbia, South Carolina 29208}

\newcommand*{\NOWFIU }{ Florida International University, Miami, Florida 33199}

\newcommand*{\NOWOHIOU }{ Ohio University, Athens, Ohio  45701}

\newcommand*{\NOWCMU }{ Carnegie Mellon University, Pittsburgh, Pennsylvania 15213}

\newcommand*{\NOWINDSTRA }{ Systems Planning and Analysis, Alexandria, Virginia 22311}

\newcommand*{\NOWASU }{ Arizona State University, Tempe, Arizona 85287-1504}

\newcommand*{\NOWCISCO }{ Cisco, Washington, DC 20052}

\newcommand*{\NOWUK }{ University of Kentucky, LEXINGTON, KENTUCKY 40506}

\newcommand*{\NOWINFNFR }{ INFN, Laboratori Nazionali di Frascati, Frascati, Italy}

\newcommand*{\NOWUNCW }{ North Carolina}

\newcommand*{\NOWHAMPTON }{ Hampton University, Hampton, VA 23668}

\newcommand*{\NOWTulane }{ Tulane University, New Orleans, Lousiana  70118}

\newcommand*{\NOWKYUNGPOOK }{ Kungpook National University, Taegu 702-701, South Korea}

\newcommand*{\NOWCUA }{ Catholic University of America, Washington, D.C. 20064}

\newcommand*{\NOWGEORGETOWN }{ Georgetown University, Washington, DC 20057}

\newcommand*{\NOWJMU }{ James Madison University, Harrisonburg, Virginia 22807}

\newcommand*{\NOWCALTECH }{ California Institute of Technology, Pasadena, California 91125}

\newcommand*{\NOWMOSCOW }{ Moscow State University, General Nuclear Physics Institute, 119899 Moscow, Russia}

\newcommand*{\NOWVIRGINIA }{ University of Virginia, Charlottesville, Virginia 22901}

\newcommand*{\NOWYEREVAN }{ Yerevan Physics Institute, 375036 Yerevan, Armenia}

\newcommand*{\NOWRICE }{ Rice University, Houston, Texas 77005-1892}

\newcommand*{\NOWBATES }{ MIT-Bates Linear Accelerator Center, Middleton, MA 01949}

\newcommand*{\NOWODU }{ Old Dominion University, Norfolk, Virginia 23529}

\newcommand*{\NOWVSU }{ Virginia State University, Petersburg,Virginia 23806}

\newcommand*{\NOWORST }{ Oregon State University, Corvallis, Oregon 97331-6507}

\newcommand*{\NOWGWU }{ The George Washington University, Washington, DC 20052}

\newcommand*{\NOWMIT }{ Massachusetts Institute of Technology, Cambridge, Massachusetts  02139-4307}

\newcommand*{\NOWINFNGE }{ INFN, Sezione di Genova, 16146 Genova, Italy}


\newcommand*{\NOWdeceased }{ Deceased}

%%%%%%%%%%%%%%%%%%%% authors %%%%%%%%% 
%vpk,lg,dw,paul stoler, m. battaglieri, r. devita,g. adams, j.li,m.nozar,c.salgado  
\author{V.~Kubarovsky}
     \affiliation{\RPI}\affiliation{\JLAB}
\author{L.~Guo}
     \affiliation{\VANDER}
\author{D.P.~Weygand}
     \affiliation{\JLAB}
\author{P.~Stoler}
     \affiliation{\RPI}
\author{M.~Battaglieri}
     \affiliation{\INFNGE}
\author{R.~DeVita}
     \affiliation{\INFNGE}
\author{G.~Adams}
     \affiliation{\RPI}
\author{Ji~Li}
     \affiliation{\RPI}
\author{M.~Nozar}
     \affiliation{\JLAB}
     \altaffiliation{\NONE}
\author{C.~Salgado}
     \affiliation{\NSU}
\author{P.~Ambrozewicz}
     \affiliation{\FIU}
\author{E.~Anciant}
     \affiliation{\SACLAY}
\author{M.~Anghinolfi}
     \affiliation{\INFNGE}
\author{B.~Asavapibhop}
     \affiliation{\UMASS}
\author{G.~Audit}
     \affiliation{\SACLAY}
\author{T.~Auger}
     \affiliation{\SACLAY}
\author{H.~Avakian}
     \affiliation{\JLAB}
     \altaffiliation{\INFNFR}
\author{H.~Bagdasaryan}
     \affiliation{\ODU}
\author{J.P.~Ball}
     \affiliation{\ASU}
\author{S.~Barrow}
     \affiliation{\FSU}
\author{K.~Beard}
     \affiliation{\JMU}
\author{M.~Bektasoglu}
     \affiliation{\OHIOU}
     \altaffiliation{\KYUNGPOOK}
\author{M.~Bellis}
     \affiliation{\RPI}
\author{N.~Benmouna}
     \affiliation{\GWU}
\author{B.L.~Berman}
     \affiliation{\GWU}
\author{N.~Bianchi}
     \affiliation{\INFNFR}
\author{A.S.~Biselli}
     \affiliation{\CMU}
     \altaffiliation{\RPI}
\author{S.~Boiarinov}
     \affiliation{\ITEP}
      \altaffiliation[Current address:]{\NOWJLAB}
\author{B.E.~Bonner}
     \affiliation{\RICE}
\author{S.~Bouchigny}
     \affiliation{\ORSAY}
     \altaffiliation{\JLAB}
\author{R.~Bradford}
     \affiliation{\CMU}
\author{D.~Branford}
     \affiliation{\ECOSSEE}
\author{W.J.~Briscoe}
     \affiliation{\GWU}
\author{W.K.~Brooks}
     \affiliation{\JLAB}
\author{V.D.~Burkert}
     \affiliation{\JLAB}
\author{C.~Butuceanu}
     \affiliation{\WM}
\author{J.R.~Calarco}
     \affiliation{\UNH}
\author{G.P.~Capitani}
     \affiliation{\INFNFR}
\author{D.S.~Carman}
     \affiliation{\CMU}
      \altaffiliation[Current address:]{\NOWOHIOU}
\author{B.~Carnahan}
     \affiliation{\CUA}
\author{C.~Cetina}
     \affiliation{\GWU}
      \altaffiliation[Current address:]{\NOWCMU}
\author{S.~Chen}
     \affiliation{\FSU}
\author{L.~Ciciani}
     \affiliation{\ODU}
\author{P.L.~Cole}
     \affiliation{\UTEP}
     \altaffiliation{\JLAB}
\author{A.~Coleman}
     \affiliation{\WM}
      \altaffiliation[Current address:]{\NOWINDSTRA}
\author{J.~Connelly}
     \affiliation{\GWU}
      \altaffiliation[Current address:]{\NOWCISCO}
\author{D.~Cords}
%      \altaffiliation[Current address:]{\NOWdeceased}
      \altaffiliation{\NOWdeceased}
     \affiliation{\JLAB}
\author{P.~Corvisiero}
     \affiliation{\INFNGE}
\author{D.~Crabb}
     \affiliation{\VIRGINIA}
\author{H.~Crannell}
     \affiliation{\CUA}
\author{J.P.~Cummings}
     \affiliation{\RPI}
\author{E.~De~Sanctis}
     \affiliation{\INFNFR}
\author{R.~DeVita}
     \affiliation{\INFNGE}
\author{P.V.~Degtyarenko}
     \affiliation{\JLAB}
     \altaffiliation{\ITEP}
\author{H.~Denizli}
     \affiliation{\PITT}
\author{L.~Dennis}
     \affiliation{\FSU}
\author{K.V.~Dharmawardane}
     \affiliation{\ODU}
\author{K.S.~Dhuga}
     \affiliation{\GWU}
\author{C.~Djalali}
     \affiliation{\SCAROLINA}
\author{G.E.~Dodge}
     \affiliation{\ODU}
\author{D.~Doughty}
     \affiliation{\CNU}
     \altaffiliation{\JLAB}
\author{P.~Dragovitsch}
     \affiliation{\FSU}
\author{M.~Dugger}
     \affiliation{\ASU}
\author{S.~Dytman}
     \affiliation{\PITT}
\author{O.P.~Dzyubak}
     \affiliation{\SCAROLINA}
\author{M.~Eckhause}
     \affiliation{\WM}
\author{H.~Egiyan}
     \affiliation{\JLAB}
     \altaffiliation{\WM}
\author{K.S.~Egiyan}
     \affiliation{\YEREVAN}
\author{L.~Elouadrhiri}
     \affiliation{\CNU}
     \altaffiliation{\JLAB}
\author{A.~Empl}
     \affiliation{\RPI}
\author{P.~Eugenio}
     \affiliation{\FSU}
\author{L.~Farhi}
     \affiliation{\SACLAY}
\author{R.~Fatemi}
     \affiliation{\VIRGINIA}
\author{R.J.~Feuerbach}
     \affiliation{\CMU}
\author{J.~Ficenec}
     \affiliation{\VT}
\author{T.A.~Forest}
     \affiliation{\ODU}
\author{V.~Frolov}
     \affiliation{\RPI}
\author{H.~Funsten}
     \affiliation{\WM}
\author{S.J.~Gaff}
     \affiliation{\DUKE}
\author{M.~Gar\c{c}on}
     \affiliation{\SACLAY}
\author{G.~Gavalian}
     \affiliation{\UNH}
     \altaffiliation{\YEREVAN}
\author{G.P.~Gilfoyle}
     \affiliation{\URICH}
\author{K.L.~Giovanetti}
     \affiliation{\JMU}
\author{P.~Girard}
     \affiliation{\SCAROLINA}
\author{R.~Gothe}
     \affiliation{\SCAROLINA}
\author{C.I.O.~Gordon}
     \affiliation{\ECOSSEG}
\author{K.~Griffioen}
     \affiliation{\WM}
\author{M.~Guidal}
     \affiliation{\ORSAY}
\author{M.~Guillo}
     \affiliation{\SCAROLINA}
\author{V.~Gyurjyan}
     \affiliation{\JLAB}
\author{C.~Hadjidakis}
     \affiliation{\ORSAY}
\author{R.S.~Hakobyan}
     \affiliation{\CUA}
\author{D.~Hancock}
     \affiliation{\WM}
      \altaffiliation[Current address:]{\NOWTulane}
\author{J.~Hardie}
     \affiliation{\CNU}
     \altaffiliation{\JLAB}
\author{D.~Heddle}
     \affiliation{\CNU}
     \altaffiliation{\JLAB}
\author{P.~Heimberg}
     \affiliation{\GWU}
\author{F.W.~Hersman}
     \affiliation{\UNH}
\author{K.~Hicks}
     \affiliation{\OHIOU}
\author{R.S.~Hicks}
     \affiliation{\UMASS}
\author{M.~Holtrop}
     \affiliation{\UNH}
\author{J.~Hu}
     \affiliation{\RPI}
\author{C.E.~Hyde-Wright}
     \affiliation{\ODU}
\author{Y.~Ilieva}
     \affiliation{\GWU}
\author{M.M.~Ito}
     \affiliation{\JLAB}
\author{D.~Jenkins}
     \affiliation{\VT}
\author{K.~Joo}
     \affiliation{\UCONN}
     \altaffiliation{\VIRGINIA}
\author{H.G.~Juengst}
     \affiliation{\GWU}
\author{J.H.~Kelley}
     \affiliation{\DUKE}
\author{M.~Khandaker}
     \affiliation{\NSU}
\author{D.H.~Kim}
     \affiliation{\KYUNGPOOK}
\author{K.Y.~Kim}
     \affiliation{\PITT}
\author{K.~Kim}
     \affiliation{\KYUNGPOOK}
\author{M.S.~Kim}
     \affiliation{\KYUNGPOOK}
\author{W.~Kim}
     \affiliation{\KYUNGPOOK}
\author{A.~Klein}
     \affiliation{\ODU}
\author{F.J.~Klein}
     \affiliation{\JLAB}
      \altaffiliation[Current address:]{\NOWCUA}
\author{A.V.~Klimenko}
     \affiliation{\ODU}
\author{M.~Klusman}
     \affiliation{\RPI}
\author{M.~Kossov}
     \affiliation{\ITEP}
\author{L.H.~Kramer}
     \affiliation{\FIU}
     \altaffiliation{\JLAB}
\author{Y.~Kuang}
     \affiliation{\WM}
\author{S.E.~Kuhn}
     \affiliation{\ODU}
\author{J.~Kuhn}
     \affiliation{\CMU}
\author{J.~Lachniet}
     \affiliation{\CMU}
\author{J.M.~Laget}
     \affiliation{\SACLAY}
\author{J.~Langheinrich}
     \affiliation{\SCAROLINA}
\author{D.~Lawrence}
     \affiliation{\UMASS}
     \altaffiliation{\ASU}
\author{A.~Longhi}
     \affiliation{\CUA}
\author{K.~Lukashin}
     \affiliation{\JLAB}
      \altaffiliation[Current address:]{\NOWCUA}
\author{W.~Major}
     \affiliation{\URICH}
\author{J.J.~Manak}
     \affiliation{\JLAB}
\author{C.~Marchand}
     \affiliation{\SACLAY}
\author{L.C.~Maximon}
     \affiliation{\GWU}
\author{S.~McAleer}
     \affiliation{\FSU}
\author{J.W.C.~McNabb}
     \affiliation{\CMU}
\author{B.A.~Mecking}
     \affiliation{\JLAB}
\author{S.~Mehrabyan}
     \affiliation{\PITT}
\author{J.J.~Melone}
     \affiliation{\ECOSSEG}
\author{M.D.~Mestayer}
     \affiliation{\JLAB}
\author{C.A.~Meyer}
     \affiliation{\CMU}
\author{K.~Mikhailov}
     \affiliation{\ITEP}
\author{R.~Minehart}
     \affiliation{\VIRGINIA}
\author{M.~Mirazita}
     \affiliation{\INFNFR}
\author{R.~Miskimen}
     \affiliation{\UMASS}
\author{V.~Mokeev}
     \affiliation{\NOWMOSCOW}
\author{L.~Morand}
     \affiliation{\SACLAY}
\author{S.A.~Morrow}
     \affiliation{\SACLAY}
     \altaffiliation{\ORSAY}
\author{M.U.~Mozer}
     \affiliation{\OHIOU}
\author{V.~Muccifora}
     \affiliation{\INFNFR}
\author{J.~Mueller}
     \affiliation{\PITT}
\author{L.Y.~Murphy}
     \affiliation{\GWU}
\author{G.S.~Mutchler}
     \affiliation{\RICE}
\author{J.~Napolitano}
     \affiliation{\RPI}
\author{R.~Nasseripour}
     \affiliation{\FIU}
\author{S.O.~Nelson}
     \affiliation{\DUKE}
\author{S.~Niccolai}
     \affiliation{\GWU}
\author{G.~Niculescu}
     \affiliation{\OHIOU}
\author{I.~Niculescu}
     \affiliation{\JMU}
     \altaffiliation{\GWU}
\author{B.B.~Niczyporuk}
     \affiliation{\JLAB}
\author{R.A.~Niyazov}
     \affiliation{\ODU}
\author{J.T.~O'Brien}
     \affiliation{\CUA}
\author{G.V.~O'Rielly}
     \affiliation{\GWU}
\author{A.K.~Opper}
     \affiliation{\OHIOU}
\author{M.~Osipenko}
     \affiliation{\INFNGE}
      \altaffiliation[Current address:]{\NOWMOSCOW}
\author{K.~Park}
     \affiliation{\KYUNGPOOK}
\author{E.~Pasyuk}
     \affiliation{\ASU}
\author{G.~Peterson}
     \affiliation{\UMASS}
\author{S.A.~Philips}
     \affiliation{\GWU}
\author{N.~Pivnyuk}
     \affiliation{\ITEP}
\author{D.~Pocanic}
     \affiliation{\VIRGINIA}
\author{O.~Pogorelko}
     \affiliation{\ITEP}
\author{E.~Polli}
     \affiliation{\INFNFR}
\author{S.~Pozdniakov}
     \affiliation{\ITEP}
\author{B.M.~Preedom}
     \affiliation{\SCAROLINA}
\author{J.W.~Price}
     \affiliation{\UCLA}
     \altaffiliation{\RPI}
\author{Y.~Prok}
     \affiliation{\VIRGINIA}
\author{D.~Protopopescu}
     \affiliation{\ECOSSEG}
\author{L.M.~Qin}
     \affiliation{\ODU}
\author{B.A.~Raue}
     \affiliation{\FIU}
     \altaffiliation{\JLAB}
\author{G.~Riccardi}
     \affiliation{\FSU}
\author{G.~Ricco}
     \affiliation{\INFNGE}
\author{M.~Ripani}
     \affiliation{\INFNGE}
\author{B.G.~Ritchie}
     \affiliation{\ASU}
\author{F.~Ronchetti}
     \affiliation{\INFNFR}
     \altaffiliation{\ROMA}
\author{P.~Rossi}
     \affiliation{\INFNFR}
\author{D.~Rowntree}
     \affiliation{\MIT}
\author{P.D.~Rubin}
     \affiliation{\URICH}
\author{F.~Sabati\'e}
     \affiliation{\SACLAY}
     \altaffiliation{\ODU}
\author{K.~Sabourov}
     \affiliation{\DUKE}
\author{J.P.~Santoro}
     \affiliation{\VT}
     \altaffiliation{\JLAB}
\author{M.~Sanzone-Arenhovel}
     \affiliation{\INFNGE}
\author{V.~Sapunenko}
     \affiliation{\INFNGE}
\author{M.~Sargsyan}
     \affiliation{\FIU}
     \altaffiliation{\JLAB}
\author{R.A.~Schumacher}
     \affiliation{\CMU}
\author{V.S.~Serov}
     \affiliation{\ITEP}
\author{A.~Shafi}
     \affiliation{\GWU}
\author{Y.G.~Sharabian}
     \affiliation{\YEREVAN}
      \altaffiliation[Current address:]{\NOWJLAB}
\author{J.~Shaw}
     \affiliation{\UMASS}
\author{S.~Simionatto}
     \affiliation{\GWU}
\author{A.V.~Skabelin}
     \affiliation{\MIT}
\author{E.S.~Smith}
     \affiliation{\JLAB}
\author{T.~Smith}
     \affiliation{\UNH}
      \altaffiliation[Current address:]{\NOWBATES}
\author{L.C.~Smith}
     \affiliation{\VIRGINIA}
\author{D.I.~Sober}
     \affiliation{\CUA}
\author{M.~Spraker}
     \affiliation{\DUKE}
\author{A.~Stavinsky}
     \affiliation{\ITEP}
\author{S.~Stepanyan}
     \affiliation{\YEREVAN}
      \altaffiliation[Current address:]{\NOWODU}
\author{I.I.~Strakovsky}
     \affiliation{\GWU}
\author{S.~Strauch}
     \affiliation{\GWU}
\author{M.~Taiuti}
     \affiliation{\INFNGE}
\author{S.~Taylor}
     \affiliation{\RICE}
\author{D.J.~Tedeschi}
     \affiliation{\SCAROLINA}
     \altaffiliation{\PITT}
\author{U.~Thoma}
     \affiliation{\JLAB}
     \altaffiliation{\BONN}
\author{R.~Thompson}
     \affiliation{\PITT}
\author{L.~Todor}
     \affiliation{\CMU}
\author{C.~Tur}
     \affiliation{\SCAROLINA}
\author{M.~Ungaro}
     \affiliation{\RPI}
\author{M.F.~Vineyard}
     \affiliation{\UNIONC}
     \altaffiliation{\URICH}
\author{A.V.~Vlassov}
     \affiliation{\ITEP}
\author{K.~Wang}
     \affiliation{\VIRGINIA}
\author{L.B.~Weinstein}
     \affiliation{\ODU}
\author{A.~Weisberg}
     \affiliation{\OHIOU}
\author{H.~Weller}
     \affiliation{\DUKE}
\author{C.S.~Whisnant}
     \affiliation{\SCAROLINA}
      \altaffiliation[Current address:]{\NOWJMU}
\author{E.~Wolin}
     \affiliation{\JLAB}
\author{M.H.~Wood}
     \affiliation{\SCAROLINA}
\author{A.~Yegneswaran}
     \affiliation{\JLAB}
\author{J.~Yun}
     \affiliation{\ODU}
 

\collaboration{The CLAS Collaboration}
     \noaffiliation
% 
 
%The Southeastern Universities Research Association (SURA) operates the 
%Thomas Jefferson National Accelerator Facility for the United States 
%Department of Energy under contract DE-AC05-84ER40150. 
% 
% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% FOLLOWING A GENERIC TAIL FOR TEX
%   Nothing here relates to author list
%   Suggestion for acknowlegements.  Could be deleted.
%%%%\date{\today}
%%%%\begin{abstract}

 
 
 
%%%%\end{abstract}
%%%%\maketitle
%%%%\end{document}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%  Author by Institute %%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%  no of authors =224
%%%%%%  institute %%%%%%%%%%%RPI
%%     G.~Adams                      RPI
%%     M.~Bellis                      RPI
%%     J.P.~Cummings                      RPI
%%     A.~Empl                      RPI
%%     V.~Frolov                      RPI
%%     J.~Hu                      RPI
%%     M.~Klusman                      RPI
%%     Ji~Li                      RPI
%%     J.~Napolitano                      RPI
%%     P.~Stoler                      RPI
%%     M.~Ungaro                      RPI
%%     M.~Witkowski                      RPI
%%%%%%  institute %%%%%%%%%%%FIU
%%     P.~Ambrozewicz                      FIU
%%     L.H.~Kramer                      FIU
%%     R.~Nasseripour                      FIU
%%     B.A.~Raue                      FIU
%%     M.~Sargsyan                      FIU
%%%%%%  institute %%%%%%%%%%%SACLAY
%%     E.~Anciant                      SACLAY
%%     G.~Audit                      SACLAY
%%     T.~Auger                      SACLAY
%%     L.~Farhi                      SACLAY
%%     J.M.~Laget                      SACLAY
%%     C.~Marchand                      SACLAY
%%     L.~Morand                      SACLAY
%%     S.A.~Morrow                      SACLAY
%%     F.~Sabati\'e                      SACLAY
%%%%%%  institute %%%%%%%%%%%INFNGE
%%     M.~Anghinolfi                      INFNGE
%%     M.~Battaglieri                      INFNGE
%%     P.~Corvisiero                      INFNGE
%%     R.~DeVita                      INFNGE
%%     M.~Osipenko                      INFNGE
%%     G.~Ricco                      INFNGE
%%     M.~Ripani                      INFNGE
%%     M.~Sanzone-Arenhovel                      INFNGE
%%     V.~Sapunenko                      INFNGE
%%     M.~Taiuti                      INFNGE
%%%%%%  institute %%%%%%%%%%%UMASS
%%     B.~Asavapibhop                      UMASS
%%     R.S.~Hicks                      UMASS
%%     D.~Lawrence                      UMASS
%%     R.~Miskimen                      UMASS
%%     G.~Peterson                      UMASS
%%     J.~Shaw                      UMASS
%%%%%%  institute %%%%%%%%%%%JLAB
%%     H.~Avakian                      JLAB
%%     W.K.~Brooks                      JLAB
%%     V.D.~Burkert                      JLAB
%%     P.V.~Degtyarenko                      JLAB
%%     H.~Egiyan                      JLAB
%%     L.~Guo                      JLAB
%%     V.~Gyurjyan                      JLAB
%%     M.M.~Ito                      JLAB
%%     F.J.~Klein                      JLAB
%%     K.~Lukashin                      JLAB
%%     J.J.~Manak                      JLAB
%%     B.A.~Mecking                      JLAB
%%     M.D.~Mestayer                      JLAB
%%     B.B.~Niczyporuk                      JLAB
%%     M.~Nozar                      JLAB
%%     E.S.~Smith                      JLAB
%%     U.~Thoma                      JLAB
%%     D.P.~Weygand                      JLAB
%%     E.~Wolin                      JLAB
%%     A.~Yegneswaran                      JLAB
%%%%%%  institute %%%%%%%%%%%INFNFR
%%     N.~Bianchi                      INFNFR
%%     G.P.~Capitani                      INFNFR
%%     E.~DeSanctis                      INFNFR
%%     M.~Mirazita                      INFNFR
%%     V.~Muccifora                      INFNFR
%%     E.~Polli                      INFNFR
%%     F.~Ronchetti                      INFNFR
%%     P.~Rossi                      INFNFR
%%%%%%  institute %%%%%%%%%%%ODU
%%     H.~Bagdasaryan                      ODU
%%     L.~Ciciani                      ODU
%%     K.V.~Dharmawardane                      ODU
%%     G.E.~Dodge                      ODU
%%     T.A.~Forest                      ODU
%%     C.E.~Hyde-Wright                      ODU
%%     A.~Klein                      ODU
%%     A.V.~Klimenko                      ODU
%%     S.E.~Kuhn                      ODU
%%     R.A.~Niyazov                      ODU
%%     L.M.~Qin                      ODU
%%     L.B.~Weinstein                      ODU
%%     J.~Yun                      ODU
%%%%%%  institute %%%%%%%%%%%ASU
%%     J.P.~Ball                      ASU
%%     M.~Dugger                      ASU
%%     E.~Pasyuk                      ASU
%%     B.G.~Ritchie                      ASU
%%%%%%  institute %%%%%%%%%%%FSU
%%     S.~Barrow                      FSU
%%     S.~Chen                      FSU
%%     L.~Dennis                      FSU
%%     P.~Dragovitsch                      FSU
%%     P.~Eugenio                      FSU
%%     S.~McAleer                      FSU
%%     G.~Riccardi                      FSU
%%%%%%  institute %%%%%%%%%%%JMU
%%     K.~Beard                      JMU
%%     K.L.~Giovanetti                      JMU
%%     I.~Niculescu                      JMU
%%%%%%  institute %%%%%%%%%%%OHIOU
%%     M.~Bektasoglu                      OHIOU
%%     K.~Hicks                      OHIOU
%%     M.U.~Mozer                      OHIOU
%%     G.~Niculescu                      OHIOU
%%     A.K.~Opper                      OHIOU
%%     A.~Weisberg                      OHIOU
%%%%%%  institute %%%%%%%%%%%KYUNGPOOK
%%     D.H.~Kim                      KYUNGPOOK
%%     K.~Kim                      KYUNGPOOK
%%     M.S.~Kim                      KYUNGPOOK
%%     W.~Kim                      KYUNGPOOK
%%     K.~Park                      KYUNGPOOK
%%%%%%  institute %%%%%%%%%%%GWU
%%     N.~Benmouna                      GWU
%%     B.L.~Berman                      GWU
%%     W.J.~Briscoe                      GWU
%%     C.~Cetina                      GWU
%%     J.~Connelly                      GWU
%%     K.S.~Dhuga                      GWU
%%     P.~Heimberg                      GWU
%%     Y.~Ilieva                      GWU
%%     H.G.~Juengst                      GWU
%%     L.C.~Maximon                      GWU
%%     L.Y.~Murphy                      GWU
%%     S.~Niccolai                      GWU
%%     G.V.~O'Rielly                      GWU
%%     S.A.~Philips                      GWU
%%     A.~Shafi                      GWU
%%     S.~Simionatto                      GWU
%%     I.I.~Strakovsky                      GWU
%%     S.~Strauch                      GWU
%%%%%%  institute %%%%%%%%%%%CMU
%%     A.S.~Biselli                      CMU
%%     R.~Bradford                      CMU
%%     D.S.~Carman                      CMU
%%     R.J.~Feuerbach                      CMU
%%     J.~Kuhn                      CMU
%%     J.~Lachniet                      CMU
%%     J.W.C.~McNabb                      CMU
%%     C.A.~Meyer                      CMU
%%     R.A.~Schumacher                      CMU
%%     L.~Todor                      CMU
%%%%%%  institute %%%%%%%%%%%ITEP
%%     S.~Boiarinov                      ITEP
%%     M.~Kossov                      ITEP
%%     K.~Mikhailov                      ITEP
%%     N.~Pivnyuk                      ITEP
%%     O.~Pogorelko                      ITEP
%%     S.~Pozdniakov                      ITEP
%%     V.S.~Serov                      ITEP
%%     A.~Stavinsky                      ITEP
%%     A.V.~Vlassov                      ITEP
%%%%%%  institute %%%%%%%%%%%RICE
%%     B.E.~Bonner                      RICE
%%     G.S.~Mutchler                      RICE
%%     S.~Taylor                      RICE
%%%%%%  institute %%%%%%%%%%%ORSAY
%%     S.~Bouchigny                      ORSAY
%%     M.~Guidal                      ORSAY
%%     C.~Hadjidakis                      ORSAY
%%%%%%  institute %%%%%%%%%%%ECOSSEE
%%     D.~Branford                      ECOSSEE
%%%%%%  institute %%%%%%%%%%%WM
%%     C.~Butuceanu                      WM
%%     A.~Coleman                      WM
%%     M.~Eckhause                      WM
%%     H.~Funsten                      WM
%%     K.~Griffioen                      WM
%%     D.~Hancock                      WM
%%     Y.~Kuang                      WM
%%%%%%  institute %%%%%%%%%%%UNH
%%     J.R.~Calarco                      UNH
%%     G.~Gavalian                      UNH
%%     F.W.~Hersman                      UNH
%%     M.~Holtrop                      UNH
%%     T.~Smith                      UNH
%%%%%%  institute %%%%%%%%%%%CUA
%%     B.~Carnahan                      CUA
%%     H.~Crannell                      CUA
%%     R.S.~Hakobyan                      CUA
%%     A.~Longhi                      CUA
%%     J.T.~O'Brien                      CUA
%%     D.I.~Sober                      CUA
%%%%%%  institute %%%%%%%%%%%UTEP
%%     P.L.~Cole                      UTEP
%%%%%%  institute %%%%%%%%%%%deceased
%%     D.~Cords                      deceased
%%%%%%  institute %%%%%%%%%%%VIRGINIA
%%     D.~Crabb                      VIRGINIA
%%     R.~Fatemi                      VIRGINIA
%%     R.~Minehart                      VIRGINIA
%%     D.~Pocanic                      VIRGINIA
%%     Y.~Prok                      VIRGINIA
%%     L.C.~Smith                      VIRGINIA
%%     K.~Wang                      VIRGINIA
%%%%%%  institute %%%%%%%%%%%PITT
%%     H.~Denizli                      PITT
%%     S.~Dytman                      PITT
%%     K.Y.~Kim                      PITT
%%     S.~Mehrabyan                      PITT
%%     J.~Mueller                      PITT
%%     R.~Thompson                      PITT
%%%%%%  institute %%%%%%%%%%%SCAROLINA
%%     C.~Djalali                      SCAROLINA
%%     O.P.~Dzyubak                      SCAROLINA
%%     P.~Girard                      SCAROLINA
%%     M.~Guillo                      SCAROLINA
%%     J.~Langheinrich                      SCAROLINA
%%     B.M.~Preedom                      SCAROLINA
%%     D.J.~Tedeschi                      SCAROLINA
%%     C.~Tur                      SCAROLINA
%%     C.S.~Whisnant                      SCAROLINA
%%     M.H.~Wood                      SCAROLINA
%%%%%%  institute %%%%%%%%%%%CNU
%%     D.~Doughty                      CNU
%%     L.~Elouadrhiri                      CNU
%%     J.~Hardie                      CNU
%%     D.~Heddle                      CNU
%%%%%%  institute %%%%%%%%%%%YEREVAN
%%     K.S.~Egiyan                      YEREVAN
%%     Y.G.~Sharabian                      YEREVAN
%%     S.~Stepanyan                      YEREVAN
%%%%%%  institute %%%%%%%%%%%VT
%%     J.~Ficenec                      VT
%%     D.~Jenkins                      VT
%%     J.P.~Santoro                      VT
%%%%%%  institute %%%%%%%%%%%DUKE
%%     S.J.~Gaff                      DUKE
%%     J.H.~Kelley                      DUKE
%%     S.O.~Nelson                      DUKE
%%     K.~Sabourov                      DUKE
%%     M.~Spraker                      DUKE
%%     H.~Weller                      DUKE
%%%%%%  institute %%%%%%%%%%%URICH
%%     G.P.~Gilfoyle                      URICH
%%     W.~Major                      URICH
%%     P.D.~Rubin                      URICH
%%%%%%  institute %%%%%%%%%%%ECOSSEG
%%     C.I.O.~Gordon                      ECOSSEG
%%     J.J.~Melone                      ECOSSEG
%%     D.~Protopopescu                      ECOSSEG
%%%%%%  institute %%%%%%%%%%%UCONN
%%     K.~Joo                      UCONN
%%%%%%  institute %%%%%%%%%%%NSU
%%     M.~Khandaker                      NSU
%%     C.~Salgado                      NSU
%%%%%%  institute %%%%%%%%%%%NONE
%%%%%%  institute %%%%%%%%%%%UCLA
%%     J.W.~Price                      UCLA
%%%%%%  institute %%%%%%%%%%%ROMA
%%%%%%  institute %%%%%%%%%%%MIT
%%     D.~Rowntree                      MIT
%%     A.V.~Skabelin                      MIT
%%%%%%  institute %%%%%%%%%%%BONN
%%%%%%  institute %%%%%%%%%%%UNIONC
%%     M.F.~Vineyard                      UNIONC

